Efficient Numerical Methods for Gas Network Modeling and Simulation

We study the modeling and simulation of gas pipeline networks, with a focus on fast numerical methods for the simulation of transient dynamics. The obtained mathematical model of the underlying network is represented by a nonlinear differential algebraic equation (DAE). With our modeling, we reduce the number of algebraic constraints, which correspond to the $(2,2)$ block in our semi-explicit DAE model, to the order of junction nodes in the network, where a junction node couples at least three pipelines. We can furthermore ensure that the $(1, 1)$ block of all system matrices including the Jacobian is block lower triangular by using a specific ordering of the pipes of the network. We then exploit this structure to propose an efficient preconditioner for the fast simulation of the network. We test our numerical methods on benchmark problems of (well-)known gas networks and the numerical results show the efficiency of our methods.

==> Makefile <==
# latex makefile

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)

TRG	 = $(SRC:%.tex=%.pdf)

BIB = $(SRC:%.tex=%.aux)

DVI = $(SRC:%.tex=%.dvi)

PS 	= $(SRC:%.tex=%.ps)

PDF	= $(SRC:%.tex=%.pdf)

DEP     =`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`


# DEP	= *.tex *.bib */*.tex

all: $(TRG)


$(TRG): *.tex *.bib
	pdflatex 		$(SRC)
	bibtex   		$(BIB)
	pdflatex 		$(SRC)
	pdflatex 		$(SRC)
	
.PHONY: clean
clean:
	-rm *.aux *.log *.bbl *blg

